Active Collaborative Sensing for Energy Breakdown

Residential homes constitute roughly one-fourth of the total energy usage worldwide. Providing appliance-level energy breakdown has been shown to induce positive behavioral changes that can reduce energy consumption by 15%. Existing approaches for energy breakdown either require hardware installation in every target home or demand a large set of energy sensor data available for model training. However, very few homes in the world have installed sub-meters (sensors measuring individual appliance energy); and the cost of retrofitting a home with extensive sub-metering eats into the funds available for energy saving retrofits. As a result, strategically deploying sensing hardware to maximize the reconstruction accuracy of sub-metered readings in non-instrumented homes while minimizing deployment costs becomes necessary and promising. In this work, we develop an active learning solution based on low-rank tensor completion for energy breakdown. We propose to actively deploy energy sensors to appliances from selected homes, with a goal to improve the prediction accuracy of the completed tensor with minimum sensor deployment cost. We empirically evaluate our approach on the largest public energy dataset collected in Austin, Texas, USA, from 2013 to 2017. The results show that our approach gives better performance with a fixed number of sensors installed when compared to the state-of-the-art, which is also proven by our theoretical analysis.

==> problem.tex <==
\subsection{Problem Statement}
\label{sec:prob}
In active sensor deployment, we aim to maximize the energy breakdown accuracy while minimizing the sensor deployment cost. We formally define our energy reading data as a three-way tensor, $\mathbf{E_{M \times N \times T}}$, where the elements contain energy readings from $\mathbf{M}$ homes and $\mathbf{N}$ appliances for up to  $\mathbf{T}$ months. Detailed reading is available in a cell when the corresponding appliance is monitored in that home beforehand; otherwise the reading is unknown. 
% We consider household aggregate energy as one ``special'' appliance in the tensor, as it is always available by the end of each month. 
%The active sensor deployment problem can then be viewed as an active tensor completion problem. 
There are some special structure properties of this tensor, which make the active sensor deployment problem especially challenging.

\noindent{\bf $\bullet~$ Time-series data.} In energy breakdown scenario, energy data is continuously generated and collected after every sampling cycle, e.g., monthly in Figure \ref{fig:problem}. More specifically, new data will be updated at the end of each month, and the energy tensor will grow in the ``time'' dimension. At the end of each month, new <home, appliance> pairs can be 
%selected based on the newly collected energy data 
selected according to predefined selection strategy and sensor deployment budget. Once the sensor has been installed, the energy readings of the selected pairs will be available in the next month and thereafter. 

\noindent{\bf $\bullet~$ Sensor installation.}
In sensor deployment, once the sensor is installed, the appliance readings will always be available in the future. For example, if we install $K$ sensors in January and $K$ sensors in February, we will have $K$ extra readings at the end of January and $2 \times K$ extra readings at the end of February. 

\noindent{\bf $\bullet~$ Aggregate readings.}
We view the household aggregate energy as one ``special'' appliance in the energy tensor. And with the monthly energy bills from single households, we consider it as always available in our problem.

% With the monthly electricity bills from single households, aggregate data is readily to collect. Thus, we consider it as always available in our problem.

Therefore, the active sensor deployment for energy breakdown can be naturally formalized as an active tensor completion problem. More specifically, the learning procedure is: at month $t \in [1, \mathbf{T}-1]$, based on the observed energy tensor $\mathbf{E_{\Omega} \in R^{M \times N \times t}}$ where $\mathbf{\Omega}$ represents the set of indices of observed elements, and subject to budget constraint, 
we want to install the sensors to the <home, appliance> pairs which will bring the largest reconstruction error reduction of the energy tensor in the future months.
% we want to select the most informative <home, appliance> pairs to install sensors on and get their energy readings from month $t + 1$ to $T$ so that the reconstruction error of the entire energy tensor will be minimized.
